A Reassessment of the Pantheon+ and DES 5YR Calibration Uncertainties: Dovekie

Type Ia Supernovae (SNe Ia) are crucial tools to measure the accelerating expansion of the universe, comprising thousands of SNe across multiple telescopes. Accurate measurements of cosmological parameters with SNe Ia require a robust understanding and cross-calibration of the telescopes and filters. A previous cross-calibration effort, 'Fragilistic', provided 25 photometric systems, but offered no public code or ability to add new surveys. We provide an open-source cross-calibration solution, available at https://github.com/bap37/Dovekie/ . Using the Pan-STARRs (PS1) and Gaia all-sky telescopes, we characterise the measured filters from 11 photometric systems, including CfA, PS1, Foundation, DES, CSP, SDSS, and SNLS, using published observations of field stars. For the first time, we derive uncertainties on effective filter transmissions and modify filters to match the data. With the addition of direct observations of DA white dwarfs (Boyd et al. 2025), we simultaneously cross-calibrate our zeropoints across photometric systems and propagate to cosmology. With improved uncertainties from DA WDs, we find improvements to the calibration systematic uncertainty of x1.5 for the Pantheon+ (Brout et al. 2022) sample with a new systematic photometric uncertainty = 0.016 for FlatwCDM, and modest improvements to that of the DES5YR analysis. We find good agreement with previous calibration, and show that even these small calibration changes can be amplified by up to a factor of x6 in the inferred SN Ia distances, driven by calibration sensitivity in the colour-luminosity relations and SALT training. Initial results indicate that these changes cause dmu/dz = 0.025 and change the recovered value of Omega_M in LCDM by ~0.01. These may have a potentially larger impact in w0/wa space and inferences about evolving dark energy. We pursue this calculation in an ongoing full re-analysis of DES.

==> Tables/simoffset-biases.tex <==
\begin{table}
    \centering
    \caption{A summary of the biases in simulated offsets from 100 Dovekie simulations.}
    \label{tab:simoffsetbias}
    \begin{tabular}{ccc}
Filter & ZP Bias & Significance \\
\hline
CFA3K-B & $-0.0064$ & $-0.5951$ \\
CFA3K-V & $0.0011$ & $0.1017$ \\
CFA3K-i & $-0.0001$ & $-0.006$ \\
CFA3K-r & $-0.0001$ & $-0.0069$ \\
CFA3S-B & $-0.0027$ & $-0.2499$ \\
CFA3S-I & $0.0023$ & $0.2102$ \\
CFA3S-R & $0.0011$ & $0.0966$ \\
CFA3S-V & $-0.0008$ & $-0.066$ \\
CFA4P1-B & $-0.0074$ & $-0.6983$ \\
CFA4P1-V & $-0.003$ & $-0.2698$ \\
CFA4P1-i & $0.0023$ & $0.2159$ \\
CFA4P1-r & $0.0002$ & $0.0213$ \\
CFA4P2-B & $-0.0037$ & $-0.3398$ \\
CFA4P2-V & $-0.001$ & $-0.0836$ \\
CFA4P2-i & $0.0005$ & $0.0478$ \\
CFA4P2-r & $-0.0002$ & $-0.019$ \\
CSP-B & $-0.0055$ & $-0.5144$ \\
CSP-V & $-0.0011$ & $-0.0958$ \\
CSP-g & $-0.0032$ & $-0.297$ \\
CSP-i & $0.0021$ & $0.1907$ \\
CSP-V1 & $0.0039$ & $0.3485$ \\
CSP-V2 & $-0.0011$ & $-0.0921$ \\
CSP-V3 & $-0.0001$ & $-0.0051$ \\
CSP-r & $-0.0001$ & $-0.0089$ \\
DES-g & $-0.0005$ & $-0.1784$ \\
DES-i & $0.0004$ & $0.1066$ \\
DES-r & $0.0$ & $0.03$ \\
DES-z & $-0.0001$ & $-0.0086$ \\
Foundation-g & $0.0051$ & $0.7631$ \\
Foundation-i & $0.0001$ & $0.0235$ \\
Foundation-r & $-0.0001$ & $-0.0134$ \\
Foundation-z & $-0.0001$ & $-0.0179$ \\
PS1-g & $-0.0006$ & $-0.141$ \\
PS1-i & $0.0002$ & $0.0452$ \\
PS1-r & $-0.0001$ & $-0.0156$ \\
PS1-z & $-0.0001$ & $-0.0294$ \\
PS1SN-g & $0.0039$ & $0.67$ \\
PS1SN-i & $0.0002$ & $0.0334$ \\
PS1SN-r & $-0.0003$ & $-0.0433$ \\
PS1SN-z & $0.0002$ & $0.037$ \\
SDSS-g & $-0.0002$ & $-0.0718$ \\
SDSS-i & $0.0001$ & $0.0504$ \\
SDSS-r & $-0.0002$ & $-0.042$ \\
SDSS-z & $-0.0004$ & $-0.0847$ \\
SNLS-g & $-0.0005$ & $-0.0797$ \\
SNLS-i & $-0.0$ & $-0.0014$ \\
SNLS-r & $-0.0003$ & $-0.041$ \\
SNLS-z & $-0.0001$ & $-0.0134$ \\
\end{tabular}
\end{table}

